Differentially Private Imaging via Latent Space Manipulation

There is growing concern about image privacy due to the popularity of social media and photo devices, along with increasing use of face recognition systems. However, established image de-identification techniques are either too subject to re-identification, produce photos that are insufficiently realistic, or both. To tackle this, we present a novel approach for image obfuscation by manipulating latent spaces of an unconditionally trained generative model that is able to synthesize photo-realistic facial images of high resolution. This manipulation is done in a way that satisfies the formal privacy standard of local differential privacy. To our knowledge, this is the first approach to image privacy that satisfies $\varepsilon$-differential privacy \emph{for the person.}

==> fig_fid.tex <==
\begin{figure*}[th]
\centering
\includegraphics[width=0.31\textwidth]{figures_noise_metrics_fid_1024.png}
\includegraphics[width=0.31\textwidth]{figures_noise_metrics_fid_256.png}
\includegraphics[width=0.31\textwidth]{figures_noise_metrics_fid_64.png}
\caption{Identity distance and privacy loss. 
We use Fr\'echet Inception Distance~(FID)~\cite{heusel2017gans} to measure the perceptual distance (also sometimes referred as perceptual loss or identity distance) between a query image and the generated counterpart varied by privacy parameter $\varepsilon$.
Unlike pixel-wise distance metrics, FID leverages deep features from a Inception model~\cite{szegedy2016rethinking} and is widely adopted to simulate human perception.
It shows that the perceptual distance becomes smaller as the privacy loss $\varepsilon$ increases, indicating that the less noise added, the closer the generated image to its original identity, and vice versa.
}
\label{fig:fid}
\end{figure*}



==> fig_latent_space.tex <==
\begin{figure}[th]
\centering
\includegraphics[width=0.95\linewidth]{figures_latent_space_illustration.pdf}\\
\footnotesize
\makebox[0.33\linewidth][c]{(a) Distribution of}\hfill%
\makebox[0.33\linewidth][c]{(b) Mapping from}\hfill%
\makebox[0.33\linewidth][c]{(c) Mapping from}\\
\makebox[0.33\linewidth][c]{features in training set}\hfill%
\makebox[0.33\linewidth][c]{$\ZZ$ to features}\hfill%
\makebox[0.33\linewidth][c]{$\WW$ to features}\vspace{1.5mm}\\
\caption{%
Illustrative example with two factors of variation (image features, e.g.,~masculinity and hair length).
(a) An example training set where some combination (e.g.,~long haired males) is missing.
(b) This forces the mapping from $\ZZ$ to image features to become curved so that the forbidden combination disappears in $\ZZ$ to prevent the sampling of    invalid combinations.
(c) The learned mapping from $\ZZ$ to $\WW$ is able to ``undo'' much of the warping.
}
\label{fig:latent_space_illustration}
\end{figure}


==> fig_psnr_ssim.tex <==
\begin{figure*}[th]
\centering
\includegraphics[width=0.31\textwidth]{figures_noise_metrics_psnr_1024.png}
\includegraphics[width=0.31\textwidth]{figures_noise_metrics_psnr_256.png}
\includegraphics[width=0.31\textwidth]{figures_noise_metrics_psnr_64.png}
\\
\includegraphics[width=0.31\textwidth]{figures_noise_metrics_ssim_1024.png}
\includegraphics[width=0.31\textwidth]{figures_noise_metrics_ssim_256.png}
\includegraphics[width=0.31\textwidth]{figures_noise_metrics_ssim_64.png}
\caption{Trade-offs between privacy and utility.
Peak Signal-to-Noise Ratio (PSNR) and Structural Similarity Index (SSIM) are metrics commonly used to measure image quality at pixel level, and a higher value of SSIM/PSNR indicates a lower noise level and better utility.
By varying privacy parameter $\varepsilon$ in the latent space, the pixels vary accordingly.
Note that the larger the privacy loss is, the closer the image to its original.
The trends shown in the figures align with our intuition, as presumably each latent value controls a group of pixels.
}
\label{fig:psnr_ssim}
\end{figure*}



==> fig_stylegan_arch.tex <==
\begin{figure}[th]
\centering
\includegraphics[width=0.9\linewidth]{figures_stylegan_arch.pdf}\\
\makebox[0.20\linewidth][c]{\footnotesize{(a) Traditional}}\hfill%
\makebox[0.75\linewidth][c]{\footnotesize{(b) Style-based generator}}\\
\caption{
    Architecture of GANs~\cite{karras2019style}.
}
\label{fig:stylegan_arch}
\end{figure}


==> sec_acknowledgment.tex <==
\section{Acknowledgments}\label{sec:acknowledgment}
Test \cite{li2019anonymousnet}


==> sec_preliminary.tex <==
\section{Preliminaries}\label{sec:preliminary}
In this section, we first briefly review the definition of differential privacy and related theories.
We then quickly go through the fundamentals of image editing with generative adversarial networks,
and review quantitative metrics for performance evaluation.

\subsection{Differential Privacy}\label{subsec:differential_privacy}
Dwork et al.~\cite{dwork2006calibrating} defined the notion of differential privacy. 
At a high level, differential privacy guarantees that if we release information based on two databases that differ in only one individual, the information released will be from nearly indistinguishable distributions.  In other words, one individual's data has a negligible impact on the released information. 
Hence, no meaningful information can be inferred about individuals. 
The definitions below come from their work.

\begin{definition}{
(Differential Privacy). A randomized mechanism $\mathcal{M}:\mathcal{D}\rightarrow\mathcal{R}$ with domain $\mathcal{D}$ and range $\mathcal{R}$ is $\varepsilon$-differentially private if for all $D_1, D_2 \in \mathcal{D}$ satisfying $d(D_1,D_2)=1$, and for all sets $\mathcal{S} \subseteq \mathcal{R}$ of possible outputs:
$$\Pr[\mathcal{M}(D_1) \in \mathcal{S}] \leq e^{\varepsilon} \Pr[\mathcal{M}(D_2) \in \mathcal{S}] $$}
\end{definition}

We also make use of some properties of the way differentially private mechanisms combine.
\emph{Sequential composition} states that privacy loss is additive:
If we take ``multiple looks'' at the data, the privacy budget $\varepsilon$ used is the sum of the privacy budgets $\varepsilon_i$ of each ``look''.
\begin{theorem}\label{thm_scomp} (Sequential Composition \cite{mcsherry2009differentially,dwork2009differential}) Let $\mathcal{M}_1 : \mathcal{D} \rightarrow \mathcal{R}_1$ be an $\varepsilon_1$-differentially private algorithm, and let $\mathcal{M}_2 : \mathcal{D} \rightarrow \mathcal{R}_2$ be an $\varepsilon_2$-differentially private algorithm. Then their combination, defined to be $\mathcal{M}_{1,2} : \mathcal{D} \rightarrow \mathcal{R}_1 \times \mathcal{R}_2$ by the mapping: $\mathcal{M}_{1,2}(x) = (\mathcal{M}_1(x),\mathcal{M}_2(x))$ is $\varepsilon_1+\varepsilon_2$-differentially private.
\end{theorem}

We define a database $x = (x_1, x_2, \ldots, x_n) \in \mathcal{D}^n$ as a vector that represents the dataset as a histogram. 
Each entry $x_i$ in the given vector represents the information contributed by an individual. This could be their gender, salary, or any kind of personal data.

Let $\mathcal{D}_1, \ldots, \mathcal{D}_m$ denote domains, each of which could be categorical or numerical. 
A database $D$ consists of $n$ rows, $\{X^{(1)}, X^{(2)}, \ldots, X^{(n)}\}$, where each $X^{(i)}\in \mathcal{D}_1 \times \ldots \mathcal{D}_m$.


This definition assumes a dataset of many individuals.  While this might work if a social media site were to privatize images, we envision scenarios where the image creator independently privatizes the images (e.g., within a camera.)
This is referred to as Local Differential Privacy (LDP), introduced in \cite{evfimievski2003limiting} and formally defined in \cite{kasiviswanathan2011can}.
Here, we adopt the LDP definition from \cite{erlingsson2014rappor}.
\begin{definition}{
\label{def:LDP}
(Local Differential Privacy). 
We say that a randomized mechanism $\mathcal{M}$ satisfies $\varepsilon$-Local Differential Privacy where $\varepsilon > 0$
if and only if for any input $v$ and $v'$
$$\forall y \in Range(\mathcal{M}) := \frac{Pr[\mathcal{M}(v) = y]}{Pr[\mathcal{M}(v') = y]} \le e^\varepsilon,$$
where $Range(\mathcal{M})$ denotes every possible output of mechanisms $\mathcal{M}$.
}
\end{definition}

Local Differential Privacy is equivalent to the standard definition with a database size of 1; i.e., neighboring databases are any two databases of size one, with the one element replaced with another.  Thus all theorems that apply to \emph{bounded} differential privacy ($|\mathcal{D}_1| = |\mathcal{D}_2|$) hold for local differential privacy.
\begin{theorem}\label{thm:ldpequal}
Any mechanism $\mathcal{M}$ that satisfies bounded $\varepsilon$-Differential Privacy for \emph{arbitrary} neighboring databases $\mathcal{D}_1$ and $\mathcal{D}_2$, $|\mathcal{D}_1| = |\mathcal{D}_2|$ also satisfies Local Differential Privacy.
\end{theorem}
\begin{proof}
If $\mathcal{M}$ does not satisfy Local Differential Privacy, then there exist $v, v'$ such that
$$Pr[\mathcal{M}(v) = y] > e^\varepsilon \cdot Pr[\mathcal{M}(v') = y].$$
Let $D_1 = \{v\}$, $D_2 = \{v'\}$ and $\mathcal{S} = \{y\}$. Then,
$$\Pr[\mathcal{M}(D_1) \in \mathcal{S}] >  e^{\varepsilon} \cdot \Pr[\mathcal{M}(D_2) \in \mathcal{S}].$$
This violates the definition of $\varepsilon$-Differential Privacy.
Thus, $\mathcal{M}$ has to satisfy Local Differential Privacy.
\end{proof}
The validity for \emph{arbitrary} $\mathcal{D}_1$ and $\mathcal{D}_2$ is a strict interpretation.  Imagine, for example, a mechanism $\mathcal{M}$ that adds Laplace noise from a fixed distribution $Lap((5/10)/\varepsilon)$ (see \cref{def:laplace}).  If we calculate mean over a ``course evaluation'' survey with scores from 1-5, and only calculate this if we have at least 10 responses, then this mechanism satisfies $\varepsilon$-differential privacy using the Laplace mechanism (Example 1 of \cite{dwork2006calibrating}.)  But this particular distribution does \emph{not} satisfy local differential privacy for the same database.  For local differential privacy, we need to calculate sensitivity (the impact of a single individual on the released result) somewhat more strictly.

\begin{definition}
(LDP Sensitivity). For query $f$, we define LDP sensitivity as:
$$S_L = \max\limits_{\forall v} f(v) - \min\limits_{\forall v'} f(v'). $$
\end{definition}


Dwork et al.~\cite{dwork2006calibrating} showed how to calibrate noise to the sensitivity of the function $f$ such that it satisfies $\varepsilon-$differential privacy,
specifically, noise
proportional to $Lap(0, S_L/\varepsilon)$. 
Intuitively, whenever we add noise proportional to the sensitivity of $f$, we are adding noise proportional to the maximum magnitude of changes in $f$.  To formalize this, we restate the Laplace mechanism and prove that it satisfies $\varepsilon$-differential privacy %from \cite{dwork2006calibrating}
in terms of local differential privacy.

\begin{definition}{(Laplace Distribution) The probability density function (p.d.f) of the Laplace distribution $Lap(\mu, \lambda)$ is
    $$f(x|\mu, \lambda) = \frac{1}{2\lambda} e^{-|x-\mu|/\lambda}$$
    with mean $\mu$ and standard deviation  $\sqrt{2}\lambda$.}
\end{definition}

\begin{definition}\label{def:laplace}{(Laplace Mechanism~\cite{dwork2006calibrating})
    Given query $f: \mathbb{N}^{|\mathbb{X}|} \rightarrow \mathbb{R}^k$, the Laplace mechanism is
    \begin{align*}
        M(x, f, \varepsilon) = f(x) + (Y_1 \dots Y_k),
    \end{align*}
    where $Y_i \sim Lap({S_L} / {\varepsilon})$ i.i.d.
}
\end{definition}

The Laplace mechanism has been proven to satisfy $\varepsilon$-differential privacy \cite{dwork2006calibrating}.
However, we have not found an explicit proof that it satisfies \emph{local} differential privacy.  While this is straightforward given the proof in \cite{dwork2006calibrating}, we provide a proof here for completeness.

\begin{theorem}\label{thm:Laplace-LDP}
    The Laplace mechanism $M$ satisfies $\varepsilon$-local differential privacy ($\varepsilon$-LDP).
\end{theorem}
\begin{proof}
Let $v$ and $v'$ be arbitrary inputs, $f$ is the given query, and $y \in Range(\mathcal{M})$.
\begin{align*}
    \frac{Pr[M(v, f, \varepsilon) = y]}{Pr[M(v', f, \varepsilon) = y]}
    & = \frac{Pr[Lap(S_L / \varepsilon) + f(v) = y]}{Pr[Lap(S_L / \varepsilon) + f(v') = y]} \\
    & = \frac{Pr[Lap(S_L / \varepsilon) = y - f(v)]}{Pr[Lap(S_L / \varepsilon) = y - f(v')]} \\
    & = \frac{\frac{\varepsilon}{2 \cdot S_L} exp(- \frac{|y - f(v)| \varepsilon}{S_L})}{\frac{\varepsilon}{2 \cdot S_L} exp(- \frac{|y - f(v')| \varepsilon}{S_L})} \\
    & = exp(- \frac{\varepsilon(|y - f(v)| - |y - f(v')|)}{S_L}) \\
    & \le exp(\frac{\varepsilon |f(v) - f(v')|}{S_L}) \le exp(\varepsilon)
\end{align*}
\end{proof}

\subsection{Generative Adversarial Networks}
Recently, Generative Adversarial Networks (GAN)~\cite{mirza2014conditional} have received considrable attention in image processing, due to their great potential in
producing photo-realistic images~\cite{martin2017wasserstein,li2019anonymousnet,gulrajani2017improved,berthelot2017began,zhang2018self,miyato2018spectral,karras2017progressive,brock2018large,karras2019style}.
GANs are designed as two players, $D$ and $G$, playing a minmax game with adversarial loss:
\begin{align*}
L_{adv} = \mathbb{E} [\log(D(\mathbf{x}))] + \mathbb{E} [\log(1 - D(g(\mathbf{x})))]
\end{align*}
where generator $g$ is trained to fool discriminator $D$, who tries to distinguish real from adversarial images.

\input{fig_stylegan_arch.tex}
A GAN typically takes a sampled latent code $\z$ as the input and outputs an image synthesis. 
\cref{fig:stylegan_arch} showcases the architecture of GANs.
Unlike a traditional generator~\cite{karras2017progressive} that feeds the latent code though the input layer only,
StyleGAN first maps the input to an intermediate latent space $\WW$,
which then controls the generator through adaptive instance normalization (AdaIN) at each convolution layer,
with Gaussian noise added after each convolution and before evaluating the nonlinearity.
The ``A'' above stands for a learned affine transform, and ``B'' applies learned per-channel scaling factors to the noise input.
See~\cite{karras2019style} for more details.

To make GANs applicable for real image processing, existing methods either reverse the mapping from the latent space to the image space~\cite{upchurch2017deep,zhu2016generative,ma2018invertibility,bau2019seeing,gu2019image} or learn an additional encoder
associated with the GAN training~\cite{dumoulin2016adversarially,donahue2016adversarial,zhu2019lia}. 
In \cref{sec:method}, we will present a practical framework to map real world images to latent code.

\subsection{Semantics Editing with GANs}
\label{subsec:latent_space}

Given a well-trained GAN model, the generator can be formulated as function $g: \Z\rightarrow\X$,
where $\Z\subseteq\R^{d}$ denotes the $d$-dimensional latent space,
and $\X$ stands for the image space, where each sample $\x \in \X$ contains semantic information. 
Suppose we have a semantic scoring function $f_S: \X\rightarrow\S$, where $\S\subseteq\R^m$ represents the semantic space with $m$ semantics.
We can bridge the latent space $\Z$ and the semantic space $\S$ with $\s = f_S(g(\z))$, where $\s$ and $\z$ denote the semantic scores and the sampled latent code respectively.

Based on observations, \cite{shen2019interpreting} makes an assumption that for any binary facial feature (e.g., gender or age), there exists a hyperplane in the latent space serving as the separation boundary.
The semantic remains the same when the latent code stays within the same side of the hyperplane yet turns into the opposite when across the boundary.
Given a hyperplane with a unit normal vector $\n\in\R^d$, a ``distance'' can be defined from a sample $\z$ to this hyperplane as
\begin{align}
  \dis(\n, \z)= \n^T\z.  \label{eq:distance}
\end{align}
Note that $\dis()$ is not strictly a %mathematical definition of
distance, given that it can be negative;
but it is still useful and convenient in the context.
When $\z$ lies near the boundary and moves across the hyperplane, both $\dis()$ and the semantic score vary accordingly.
The sign of $\dis()$ changes as the binary semantic attribute changes.
We therefore expect these two to be linearly dependent with
\begin{align}
  f(g(\z)) = \lambda\dis(\n,\z),  \label{eq:linear-dependency}
\end{align}
where $f()$ is the scoring function for a particular semantic, and $\lambda > 0$ is a scalar mesauring how fast the semantic varies with changing distance.
We model the semantics by the linear subspace defined by $\n$.

According to \cref{eq:linear-dependency}, to manipulate the attribute of a synthesized image, we can update the original latent code
$\z$ with $\z_{edit}=\z + \alpha \n$.
It will make the synthesis look more positive on such semantic with $\alpha>0$, since the score becomes $f(g(\z_{edit}))=f(g(\z)) + \lambda\alpha$ after editing.
Similarly, $\alpha < 0$ will make the synthesis look more negative.
\cref{fig:conditional_manipulation} demonstrates this manipulation.
We use the same idea of manipulating the attributes to satisfy $\varepsilon$-differential privacy, before synthesizing the privatized image.
The continuity and monotonicity of latent space manipulation are important for our later discussions.



==> tab_experiment.tex <==
\begin{table*}[ht]
\centering
\caption{Experimental Results ($1024 \times 1024$)}
\label{tab:experiment}
\begin{tabular}{c|ccc|ccc|ccc|ccc}
Clipping      & \multicolumn{3}{c|}{$[0.00, 1.00]$} & \multicolumn{3}{c|}{$[0.10, 0.90]$} & \multicolumn{3}{c|}{$[0.25, 0.75]$} & \multicolumn{3}{c}{$[0.40, 0.60]$} \\
\midrule
$\bm{\varepsilon}$ & PSNR   & SSIM  & FID     & PSNR   & SSIM  & FID     & PSNR   & SSIM  & FID    & PSNR   & SSIM  & FID     \\
\midrule
$10^0$        & 8.528  & 0.288 & 290.943 & 10.899 & 0.425 & 155.465 & 11.855 & 0.486 & 99.901 & 12.144 & 0.509 & 145.706 \\
$10^1$        & 8.405  & 0.279 & 293.903 & 10.964 & 0.427 & 158.256 & 11.803 & 0.485 & 97.840 & 12.131 & 0.508 & 145.600 \\
$10^2$        & 8.636  & 0.286 & 291.888 & 10.964 & 0.428 & 156.425 & 11.824 & 0.485 & 97.199 & 12.149 & 0.509 & 145.363 \\
$10^3$        & 8.536  & 0.285 & 291.754 & 10.970 & 0.430 & 152.974 & 11.927 & 0.489 & 99.073 & 12.219 & 0.512 & 145.345 \\
$10^4$        & 8.537  & 0.284 & 294.713 & 11.644 & 0.456 & 128.656 & 12.637 & 0.519 & 93.368 & 12.746 & 0.531 & 136.468 \\
$10^5$        & 8.777  & 0.297 & 289.595 & 16.460 & 0.636 & 58.225  & 15.179 & 0.607 & 73.963 & 13.240 & 0.550 & 129.920 \\
$10^6$        & 10.364 & 0.351 & 263.134 & 20.023 & 0.745 & 38.261  & 15.762 & 0.625 & 69.905 & 13.291 & 0.552 & 129.181 \\
$10^7$        & 21.212 & 0.784 & 25.344  & 20.127 & 0.747 & 37.976  & 15.773 & 0.625 & 69.720 & 13.292 & 0.552 & 129.113 \\
$10^8$        & 24.775 & 0.881 & 10.750  & 20.130 & 0.748 & 37.938  & 15.773 & 0.625 & 69.754 & 13.292 & 0.552 & 129.116 \\
$10^9$        & 24.842 & 0.883 & 10.650  & 20.130 & 0.748 & 37.947  & 15.773 & 0.625 & 69.753 & 13.292 & 0.552 & 129.119 \\
\end{tabular}
\end{table*}


==> tab_optimized_pairs.tex <==
\begin{table}[t]
\centering
\caption{Evaluation of Image Encoding}
\label{tab:optimized_pairs}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc|ccc|ccc}
\multicolumn{3}{c|}{$1024 \times 1024$} & \multicolumn{3}{c|}{$256 \times 256$} & \multicolumn{3}{c}{$64 \times 64$} \\ \midrule
PSNR         & SSIM       & FID         & PSNR        & SSIM       & FID        & PSNR       & SSIM      & FID        \\ \midrule
20.406       & 0.608      & 27.667      & 21.207      & 0.798      & 30.008     & 22.135     & 0.926     & 22.968     \\
\end{tabular}%
}
\end{table}

